Speeding Up Private Distributed Matrix Multiplication via Bivariate Polynomial Codes

We consider the problem of private distributed matrix multiplication under limited resources. Coded computation has been shown to be an effective solution in distributed matrix multiplication, both providing privacy against the workers and boosting the computation speed by efficiently mitigating stragglers. In this work, we propose the use of recently-introduced bivariate polynomial codes to further speed up private distributed matrix multiplication by exploiting the partial work done by the stragglers rather than completely ignoring them. We show that the proposed approach reduces the average computation time of private distributed matrix multiplication compared to its competitors in the literature while improving the upload communication cost and the workers' storage efficiency.

==> K5_L5_T8_m2-10_N50_varvar_shiftvar_exp100_tstep0.1.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Storage},
xmin=1.6, xmax=10.4,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Expected computation time (s)},
ymin=61.4610500000003, ymax=101.93995,
ytick style={color=black}
]
\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
2 100.1
3 100.1
4 99.3280000000004
5 82.9700000000001
6 63.4070000000002
7 63.523
8 63.5079999999998
9 63.57
10 63.3010000000003
};
\addlegendentry{Proposed}
\addplot [semithick, color1, mark=x, mark size=3, mark options={solid}]
table {%
2 100.1
3 100.1
4 100.1
5 100.099
6 97.0480000000003
7 96.9490000000004
8 83.007
9 83.1230000000002
10 71.2280000000001
};
\addlegendentry{GASP}
\end{axis}

\end{tikzpicture}


==> K5_L5_T8_m2-10_N60_varvar_shiftvar_exp100_tstep0.1.tex <==
% K=5 #5
% L=5 #10
% T=8 #3
% mem_arr = np.array([2,3,4,5,6,7,8,9,10]) 
% #max_time_mem = np.array([,5,5,5])
% 
% t_step = 1e-1
% t_stop_worst = 100
% #t_range = np.arange(t_step, t_stop, t_step)
% 
% no_of_exp = 100
% no_workers = 60
% 
% grp1 = 20
% grp2 = 20
% grp3 = 20
% 
% var_param1 = 1e-1
% var_param2 = 1e-3
% var_param3 = 1e-4
% 
% shift_param1 = 10
% shift_param2 = 10
% shift_param3 = 10


% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Storage},
xmin=1.6, xmax=10.4,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Expected computation time (s)},
ymin=21.1757, ymax=103.8583,
ytick style={color=black}
]
\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
2 100.1
3 99.9700000000001
4 65.0540000000001
5 38.834
6 25.096
7 25.173
8 24.934
9 25.042
10 25.247
};
\addlegendentry{Proposed}
\addplot [semithick, color1, mark=x, mark size=3, mark options={solid}]
table {%
2 100.1
3 100.1
4 94.3060000000004
5 94.3130000000003
6 55.627
7 55.6699999999999
8 38.927
9 38.929
10 29.67
};
\addlegendentry{GASP}
\end{axis}

\end{tikzpicture}

